Algorithmic Theory of ODEs and Sampling from Well-conditioned Logconcave Densities

Sampling logconcave functions arising in statistics and machine learning has been a subject of intensive study. Recent developments include analyses for Langevin dynamics and Hamiltonian Monte Carlo (HMC). While both approaches have dimension-independent bounds for the underlying $\mathit{continuous}$ processes under sufficiently strong smoothness conditions, the resulting discrete algorithms have complexity and number of function evaluations growing with the dimension. Motivated by this problem, in this paper, we give a general algorithm for solving multivariate ordinary differential equations whose solution is close to the span of a known basis of functions (e.g., polynomials or piecewise polynomials). The resulting algorithm has polylogarithmic depth and essentially tight runtime - it is nearly linear in the size of the representation of the solution. We apply this to the sampling problem to obtain a nearly linear implementation of HMC for a broad class of smooth, strongly logconcave densities, with the number of iterations (parallel depth) and gradient evaluations being $\mathit{polylogarithmic}$ in the dimension (rather than polynomial as in previous work). This class includes the widely-used loss function for logistic regression with incoherent weight matrices and has been subject of much study recently. We also give a faster algorithm with $ \mathit{polylogarithmic~depth}$ for the more general and standard class of strongly convex functions with Lipschitz gradient. These results are based on (1) an improved contraction bound for the exact HMC process and (2) logarithmic bounds on the degree of polynomials that approximate solutions of the differential equations arising in implementing HMC.

==> app_cal.tex <==
\section{Some dirty calculations}
\begin{lemma}
Let $x \sim {\cal N}(0,1)$, we have
\begin{align*}
\E \left[ e^{\lambda (a x + b |x|)} \right] \leq e^{\lambda^2 (b+a)^2/2}.
\end{align*}
\end{lemma}

\begin{proof}

We state a useful fact (from wolfram), for any $c$,
\begin{align*}
\frac{1}{\sqrt{2\pi}} \int_{0}^{\infty} e^{ c x }  e^{- x^2 /2 } \d x = & ~  \frac{1}{2} e^{c^2 / 2} ( \text{erf}( c / \sqrt{2} ) + 1 ).
\end{align*}
We state a another useful fact, 
\begin{align*}
\text{erf}(x) = \frac{2}{\sqrt{\pi}} ( x - \frac{1}{3} x^3 + \frac{1}{10} x^5 + O(x^6))
\end{align*}
For any $|x| \leq 1/10$, we have
\begin{align*}
\frac{2}{\sqrt{\pi}} ( x - \frac{2}{3} x^3) \geq \text{erf}(x) \geq \frac{2}{\sqrt{\pi}} ( x - \frac{1}{3} x^3 ) \implies \text{erf}(x) = \frac{2}{\sqrt{\pi}} x + O(x^3).
\end{align*}
%Further, we have
%\begin{align*}
%& ~ \frac{4}{\sqrt{\pi}} x \geq \text{erf}(x) \geq \frac{2}{\sqrt{\pi}} x \\
%\implies & ~ \frac{4}{\sqrt{ 2\pi}} x \geq \text{erf}(x / \sqrt{2}) \geq \frac{2}{\sqrt{2 \pi}} x 
%\end{align*}

We have 
\begin{align*}
 & ~ \E \left[ e^{\lambda (a x + b |x|)} \right] \\
= & ~ \frac{1}{\sqrt{2\pi}} \int_{-\infty}^{\infty} e^{\lambda ( a x + b |x|)}  e^{- x^2 /2 } \d x \\
= & ~ \frac{1}{\sqrt{2\pi}} \int_{0}^{\infty} e^{\lambda ( a x + b x)}  e^{- x^2 /2 } \d x + \frac{1}{\sqrt{2\pi}} \int_{-\infty}^{0} e^{\lambda ( a x - b x)}  e^{- x^2 /2 } \d x \\
= & ~ \frac{1}{\sqrt{2\pi}} \int_{0}^{\infty} e^{\lambda ( b + a) x }  e^{- x^2 /2 } \d x  - \frac{1}{\sqrt{2\pi}} \int_{+\infty}^{0} e^{\lambda (b - a) x}  e^{- x^2 /2 } \d x \\
= & ~ \frac{1}{\sqrt{2\pi}} \int_{0}^{\infty} e^{\lambda ( b + a) x }  e^{- x^2 /2 } \d x  + \frac{1}{\sqrt{2\pi}} \int_{0}^{+\infty} e^{\lambda (b - a) x}  e^{- x^2 /2 } \d x \\
= & ~ \frac{1}{2} e^{ \lambda^2( b + a )^2 / 2 } ( \text{erf}( \lambda(b+a) / \sqrt{2} ) + 1 ) + \frac{1}{2} e^{\lambda^2 (b-a)^2 /2} ( \text{erf} ( \lambda ( b - a ) / \sqrt{2} ) + 1 ) \\
= & ~ \frac{1}{2} e^{ \lambda^2( b + a )^2 / 2 } (1 + \frac{2}{\sqrt{2\pi}} \lambda (b + a) + O( (\lambda (b+a))^3) ) + \frac{1}{2} e^{\lambda^2 (b-a)^2 /2} ( 1 + \frac{2}{\sqrt{2\pi}} \lambda (b - a) + O( (\lambda (b-a) )^3  )
\end{align*}

\end{proof}

==> app_more.tex <==
\section{Extending $\sum_{i=1}^n \phi( a_i x )$ to $\sum_{i=1}^n \phi_i ( A_i x)$}
\tat{To be fixed..}
The general HMC dynamic.  Recall that a Hamiltonian of a simple system is written as
\begin{align*}
H(y) = H(y_1, y_2) =  \sum_{i=1}^n \phi_i (a_i^\top y_1) + \frac{1}{2} \| y_2 \|_2
\end{align*}
where $a_i \in \R^d$.

We define the general version as follows
\begin{align*}
H(y) = H(y_1, y_2) =  \sum_{i=1}^n \phi_i (A_i y_1) + \frac{1}{2} \| y_2 \|_2
\end{align*}
where $A_i \in \R^{k \times d}$ .

And we have
\begin{align}\label{eq:extending_def_d_y_1_d_y_2}
\frac{ \d }{ \d t} \begin{bmatrix} y_1 \\ y_2 \end{bmatrix}
= 
\begin{bmatrix}
y_2 \\
-G'(y_1) 
\end{bmatrix}
= 
\begin{bmatrix}
y_2 \\ 
- A^\top \phi'(A y_1)
\end{bmatrix}
\end{align}
where $A \in \R^{kn \times d}$ and $\phi'(A y_1) \in \R^{k n}$ defined as 
\begin{align*}
A = \begin{bmatrix}
A_1 \\
A_2 \\
\vdots \\
A_n
\end{bmatrix}
,
\phi'(A y_1) 
=
\begin{bmatrix}
\phi_1' (A_1 y_1) \\
\phi_2' (A_2 y_2) \\
\vdots \\
\phi_n' (A_n y_n)
\end{bmatrix}
\end{align*}
We multiply matrix $A \in \R^{kn \times d}$ on both sides of Eq.~\eqref{eq:extending_def_d_y_1_d_y_2}
\begin{align*}
\frac{ \d }{ \d t} \begin{bmatrix} A y_1 \\ A y_2 \end{bmatrix}
=
\begin{bmatrix}
A y_2 \\
- A A^\top \phi'(A y_1)
\end{bmatrix}
\end{align*}

Thus, for the assumption we still assume $\| A A^\top \|_{\infty \rightarrow \infty}$ and for the final result, we replace $n$ by $nk$ everywhere.


\begin{theorem}[Sampling]\label{thm:logistic_loss_sampling_general_A}
For each $i \in [n]$, let $A_i \in \R^{k \times d}$. Let $A = [ A_1^\top ~ A_2^\top ~ \cdots ~ A_n^\top ]^\top$. 
Let $A \in \R^{k n \times d}$ be a matrix with 
\[
\| A A^\top \|_{\infty \rightarrow \infty} = \tau,
\mathrm{~and~} I \preceq A^\top A \preceq \kappa \cdot I.
\]
Let $\phi_i :\R \rightarrow \R$ be a function s.t. $\phi'$ is $L_{\phi'}$-Lipschitz and $\phi_i$ has Cauchy estimate $M$ and radius of convergence $r$, $\forall i \in [n]$. Namely,
\begin{align*}
\forall i, \forall l, \forall a \in \R,  | \phi_i^{(l)} (a) | \leq M l! r^{-l},
\end{align*} 
 Then there exists an algorithm that samples from a density $\eps$-close to the (Strongly log-concave) density proportional to $e^{-\sum_{i=1}^n \phi_i(A_i \cdot x)}$ using 
\[
\tilde{O}( kn (\kappa + \sqrt{\tau M/r}+\sqrt{\tau L_{\phi'}}+  \sqrt{\log (kn) }/r)^2)
\]
time and $\tilde{O}(1)$ function evaluations.
\end{theorem}

\Zhao{Santosh, do you know some application of theorem?}
